Fine-Tuning Graph Neural Networks via Graph Topology induced Optimal Transport

Recently, the pretrain-finetuning paradigm has attracted tons of attention in graph learning community due to its power of alleviating the lack of labels problem in many real-world applications. Current studies use existing techniques, such as weight constraint, representation constraint, which are derived from images or text data, to transfer the invariant knowledge from the pre-train stage to fine-tuning stage. However, these methods failed to preserve invariances from graph structure and Graph Neural Network (GNN) style models. In this paper, we present a novel optimal transport-based fine-tuning framework called GTOT-Tuning, namely, Graph Topology induced Optimal Transport fine-Tuning, for GNN style backbones. GTOT-Tuning is required to utilize the property of graph data to enhance the preservation of representation produced by fine-tuned networks. Toward this goal, we formulate graph local knowledge transfer as an Optimal Transport (OT) problem with a structural prior and construct the GTOT regularizer to constrain the fine-tuned model behaviors. By using the adjacency relationship amongst nodes, the GTOT regularizer achieves node-level optimal transport procedures and reduces redundant transport procedures, resulting in efficient knowledge transfer from the pre-trained models. We evaluate GTOT-Tuning on eight downstream tasks with various GNN backbones and demonstrate that it achieves state-of-the-art fine-tuning performance for GNNs.

==> Tables/tab_datasets.tex <==
\begin{table}[th]
\def\p{$\pm$} 
\centering
\vspace{-2mm}
\caption{Test ROC-AUC (\%) of GIN backbone on downstream molecular property prediction benchmarks.(The parentheses indicate the masked matrix.)}
\setlength\tabcolsep{4pt}
\vspace{-2mm}
\scalebox{0.85}{
\begin{tabular}{c|cccc}
\toprule 
Methods & BBBP & Tox21 & Toxcast& SIDER   \\
\# BPTs & 1 & 12 & 617 & 27 \\
\# $\mathcal{A}$\_distance &  1.57 & 1.56 &1.56& 1.41 \\
\midrule
w/o MWD & 68.7$\pm$3.4 & 75.9$\pm$0.5 & 63.1$\pm$0.6 & 60.2$\pm$0.9  \\
w/ MWD$(\mbf{1}_{n\times n})$ & 66.2$\pm$3.3 & 75.3$\pm$0.9 & 63.6$\pm$0.6 & 62.7$\pm$0.7 \\
w/ MWD$(\A)$ & \textbf{69.6$\pm$2.6} & \textbf{75.7$\pm$0.5}  & {63.8$\pm$0.4}  & 63.5$\pm$0.6 \\
w/ MWD$(\mbf{I})$ &  68.6$\pm$3.5 & 75.4$\pm$0.7 & \textbf{64.1$\pm$0.3} & \textbf{63.7$\pm$0.5} \\
\midrule
 Methods & ClinTox & MUV & HIV & BACE \\
 \# BPTs & 2 & 17 & 1 & 1 \\
 \# $\mathcal{A}$\_distance & 1.41 & 1.19 & 1.65 & 1.65 \\
 \midrule
 w/o MWD &  69.5$\pm$5.0 &69.5$\pm$1.3  & 78.2$\pm$1.2 & 82.5$\pm$1.7 \\
w/ MWD$(\mbf{1}_{n\times n})$ &  69.5$\pm$5.0 & 74.3$\pm$1.3 & 78.2$\pm$0.8 & \textbf{83.7$\pm$1.9} \\
w/  MWD$(\A)$ &  \textbf{70.9$\pm$5.8} &  \textbf{80.7$\pm$0.6} & \textbf{78.5$\pm$1.5}  & 83.1$\pm$1.9\\
 w/ MWD$(\mbf{I})$ &  69.7$\pm$4.0 & 80.2$\pm$0.9 & 78.3$\pm$1.3  & 82.6$\pm$2.5 \\
\bottomrule
    \end{tabular}
    }
    \vspace{-0mm}
    \label{tab:ab_ot}    
\end{table}

==> Tables/tab_gwd_all_sup.tex <==
\begin{table*}[th]
\def\p{$\pm$} 
\setlength\tabcolsep{3pt}
\centering
\vspace{-0mm}
\caption{Test ROC-AUC (\%) of GIN(supervised\_contexpred) on downstream molecular property prediction benchmarks.}
\vspace{-3mm}
\scalebox{0.74}{
\begin{tabular}{l|cccccccc|c}
\toprule 
Methods & BBBP & Tox21 & Toxcast& SIDER & ClinTox & MUV & HIV & BACE & Avg \\
\midrule
Fine-Tuning~(baseline) & 68.7$\pm$1.3 & \textbf{78.1\p 0.6} & 65.7\p 0.6 & 62.7\p 0.8 & 72.6\p 1.5 & 81.3\p 2.1 & 79.9\p 0.7 & 84.5\p 0.7 & 74.19 \\
\midrule
L2\_SP~\cite{xuhong2018explicit} & 68.5$\pm$1.0 & 78.7$\pm$0.3 & 65.7$\pm$0.4 &	63.8$\pm$0.3 & 71.8$\pm$1.6 & 85.0$\pm$1.1 & 77.5$\pm$0.9 & 84.5$\pm$0.9 &74.44 \\
 DELTA\cite{li2018delta} & 68.4$\pm$1.2 & 77.9$\pm$0.2 & 65.6$\pm$0.2 & 62.9$\pm$0.8 & 72.7$\pm$1.9 & 85.9$\pm$1.3 & 75.6$\pm$0.4 & 79.0$\pm$1.1 & 73.50 \\
 Feature(DELTA w/o ATT) & 68.6$\pm$0.9 & 77.9$\pm$0.2 & 65.7$\pm$0.2 & 63.0$\pm$0.6 & 72.7$\pm$1.5 & 85.6$\pm$1.0 & 77.9$\pm$0.2 & 78.4$\pm$0.7 & 73.73 \\
BSS\cite{chen2019catastrophic} & 70.0$\pm$1.0 & 78.3$\pm$0.4 &  65.8$\pm$0.3 & 62.8$\pm$0.6 & 73.7$\pm$1.3 & 78.6$\pm$2.1 & 79.9$\pm$1.4 & 84.2$\pm$1.0 & 74.16 \\
StochNorm~\cite{kou2020stochastic} & 69.8$\pm$0.9 & 78.4$\pm$0.3 & 66.1$\pm$0.4 & 62.2$\pm$0.7 & 73.2$\pm$2.1 & 82.5$\pm$2.6 & 80.2$\pm$0.7 & 84.2$\pm$2.3 & 74.58 \\
\midrule
% OT &  \\
GTOT-Tuning~(Ours) & \textbf{71.5$\pm$0.8}$\uparrow_{2.8} $ & {78.6$\pm$0.3}$\uparrow_{0.5} $ & 66.6$\pm$0.4$\uparrow_{0.9}$ & 63.3$\pm$0.6$\uparrow_{0.6}$ & 77.9$\pm$3.2$\uparrow_{5.3}$ & 85.0$\pm$0.9$\uparrow_{3.7}$ & \textbf{81.1$\pm$0.5}$\uparrow_{1.2}$ & \textbf{85.3$\pm$1.5}$\uparrow_{3.8}$ &  76.16$\uparrow_{1.97}$ \\
\midrule
MGWD~(Ours) & 69.7$\pm$1.2$\uparrow_{1.8}$ & 78.6$\pm$0.3$\downarrow_{0.3}$ & 66.4$\pm$0.2$\uparrow_{0.3}$ & 63.1$\pm$0.7$\uparrow_{1.0}$ & 76.0$\pm$1.5$\uparrow_{9.4}$ & $\uparrow_{3.5}$ & $\uparrow_{1.0}$ & 85.9$\pm$0.7$\uparrow_{3.6}$ & 73.43 
\bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \label{tab:sup_GIN_molecular}    
\end{table*}


==> Tables/tab_molecular_sup_gcn.tex <==
\begin{table*}[th]
\def\p{$\pm$} 
\setlength\tabcolsep{3pt} 
\centering
\vspace{-2mm}
\caption{Test ROC-AUC (\%) of GCN with \textit{contexpred +  supervised} pretrained strategy on downstream molecular property prediction benchmarks.}
\vspace{-0mm}
\scalebox{0.74}{
\begin{tabular}{c|cccccccc|c}
\toprule 
Methods & BBBP & Tox21 & Toxcast& SIDER & ClinTox & MUV & HIV & BACE & Avg \\
\midrule
Fine-Tuning~(baseline) & 68.7$\pm$1.3 & \textbf{78.1\p 0.6} & 65.7\p 0.6 & 62.7\p 0.8 & 72.6\p 1.5 & 81.3\p 2.1 & 79.9\p 0.7 & 84.5\p 0.7 & 74.19 \\
\midrule
L2\_SP~\cite{xuhong2018explicit} & 68.5$\pm$1.0 & 78.7$\pm$0.3 & 65.7$\pm$0.4 &	63.8$\pm$0.3 & 71.8$\pm$1.6 & 85.0$\pm$1.1 & 77.5$\pm$0.9 & 84.5$\pm$0.9 &74.44 \\
Feature(DELTA w/o ATT) & 68.6$\pm$0.9 & 77.9$\pm$0.2 & 65.7$\pm$0.2 & 63.0$\pm$0.6 & & 85.6$\pm$1.0 & 77.9$\pm$0.2 & 78.4$\pm$0.7 \\
 DELTA\cite{li2018delta} & 68.4$\pm$1.2 & 77.9$\pm$0.2 &  & 62.9$\pm$0.8 & 72.7$\pm$1.9 & 85.9$\pm$1.3 & 75.6$\pm$0.4 & 79.0$\pm$1.1 \\
BSS\cite{chen2019catastrophic} & 70.0$\pm$1.0 & 78.3$\pm$0.4 &  65.8$\pm$0.3 & 62.8$\pm$0.6 & 73.7$\pm$1.3 & 78.6$\pm$2.1 & 79.9$\pm$1.4 & 84.2$\pm$1.0 & 74.16 \\
StochNorm~\cite{kou2020stochastic} & 69.8$\pm$0.9 & 78.4$\pm$0.3 & 66.1$\pm$0.4 & 62.2$\pm$0.7 & 73.2$\pm$2.1 & 82.5$\pm$2.6 & 80.2$\pm$0.7 & 84.2$\pm$2.3 & 74.58 \\
\midrule
% OT &  \\
MWD~(Ours) & \textbf{71.5$\pm$0.8}$\uparrow_{2.8} $ & {78.6$\pm$0.3}$\uparrow_{0.5} $ & 66.6$\pm$0.4$\uparrow_{0.9}$ & 63.3$\pm$0.6$\uparrow_{0.6}$ & 77.9$\pm$3.2$\uparrow_{5.3}$ & 85.0$\pm$0.9$\uparrow_{3.7}$ & \textbf{81.1$\pm$0.5}$\uparrow_{1.2}$ & \textbf{85.3$\pm$1.5}$\uparrow_{3.8}$ &  76.16$\uparrow_{1.97}$ \\
\midrule
MGWD~(Ours) & 69.7$\pm$1.2$\uparrow_{1.8}$ & 78.6$\pm$0.3$\downarrow_{0.3}$ & 66.4$\pm$0.2$\uparrow_{0.3}$ & 63.1$\pm$0.7$\uparrow_{1.0}$ & 76.0$\pm$1.5$\uparrow_{9.4}$ & $\uparrow_{3.5}$ & $\uparrow_{1.0}$ & 85.9$\pm$0.7$\uparrow_{3.6}$ & 73.43  \\
\bottomrule
    \end{tabular}
    }
    \vspace{-0mm}
    \label{tab:sup_GCN_molecular}    
\end{table*}


==> Tables/tab_sota.tex <==
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> images/fig_catastrophic_forgetting_mgwd.tex <==
\begin{figure*}[htbp]
\centering
    \subfigure{
    \begin{minipage}[s]{0.3\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{images/hiv_seed42mgwd.pdf}
    \end{minipage}%
    }%
    \quad
    \subfigure{
    \begin{minipage}[s]{0.3\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{images/hiv_seed42embeddings_distance_mgwd.pdf}
    % \caption(b)
    \end{minipage}%
    }%
    
    
% }%
\centering

\caption{Weights Distance and representation distance curves between pre-trained initialization weights and fine-tuned weights. Comparing the vanilla fine-tuning, our \textbf{GTOT-MGWD regularizer} can implicitly constrain the weights to deviate from the pre-trained parameters, alleviating the catastrophic forgetting to some extent. }
\label{fig:catastropic_forgetting_gwd}
\end{figure*}

==> images/fig_masked_wd_gwd.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{images/maskedWD_GWD.pdf}
     \caption{ An example of using masked WD and GWD on a graph. When  the mask matrix is set to the adjacency matrix of the graph, the MWD and MGWD can be rewritten as $\sum_{i}\sum_{j \in \mcal{N}(i)\bigcup\{i\}}\P_{ij}\C_{ij}$ and  $\sum_{i}\sum_{j\in\mcal{N}(i)\bigcup\{i\}} \sum_{k}\sum_{l\in\mcal{N}(k)\bigcup\{k\}}L(\C_{ik},\bar{\C}_{jl}) \P_{ij}\P_{kl}$, respectively. This implies that MGWD }
    \label{fig:maskedWD_GWD}
        \vspace{-2mm}
\end{figure}
